Towards a Theoretical Understanding of Hashing-Based Neural Nets

Parameter reduction has been an important topic in deep learning due to the ever-increasing size of deep neural network models and the need to train and run them on resource limited machines. Despite many efforts in this area, there were no rigorous theoretical guarantees on why existing neural net compression methods should work. In this paper, we provide provable guarantees on some hashing-based parameter reduction methods in neural nets. First, we introduce a neural net compression scheme based on random linear sketching (which is usually implemented efficiently via hashing), and show that the sketched (smaller) network is able to approximate the original network on all input data coming from any smooth and well-conditioned low-dimensional manifold. The sketched network can also be trained directly via back-propagation. Next, we study the previously proposed HashedNets architecture and show that the optimization landscape of one-hidden-layer HashedNets has a local strong convexity property similar to a normal fully connected neural network. We complement our theoretical results with empirical verifications.

==> app_structure.tex <==
\section{Application of Neural Subspace Embedding}
This section provides an interesting application of our oblivious neural subspace embedding result.

\subsection{Backgrounds of topology}
In this section, we introduce some backgrounds of topology.

A {\bf countable} set is a set with the same cardinality (number of elements) as some subset of the set of natural numbers. 

A topological space is called {\bf separable} if it contains a countable, dense subset; that is there exists a sequence $\{ x_n \}_{n=1}^{\infty}$ of elements of the space such that every nonempty open subset of the space contains at least one element of the sequence.

The function $f$ is said to be of class $C^{\infty}$, if it has derivatives of all orders.

The function $f$ is said to be of class $C$, if is continuous.

Let $C[-1,1]$ denote a function space.
%%%, thinking of u_m is a epsilon net.

\subsection{Using neural network to interpolate continuous function}

\begin{definition}
${\cal G}_r $ denote set $\{ \sum_{i=1}^r g_i(a_i^\top x ) ~|~ a_i \in \R^n, g_i \in C(\R), i \in [r]\}$
\end{definition}

One application of neural subspace embedding is, we can extend the result of fully connected neural network (Corollary 6.3 in \cite{p99}) to HashNets,
\begin{theorem}[Interpolation result]\label{thm:hashnet_expressive_power_formal}
Given parameter $A$, accuracy $\epsilon \in (0,1)$, failure probability $\delta \in (0,1)$, and matrix $U \in \R^{n\times d}$ with $n \gg d$. Let ${\cal P}$ denote ${\cal B}_2(A,n) \cap \mathrm{colspan}(U)$. There exist function $\phi : \R \rightarrow \R $ that are sigmoidal, strictly increasing, $L$-lipshitz and smooth, and have the property that for every $g \in {\cal G}_r$ and $\epsilon > 0$ there exist $c_i, \theta_i \in \R $ and $w_i \in \R^n$ such that, choosing a neural subspace embedding matrix $S\in \R^{s \times n}$ with $s=O(\epsilon^{-2} d A^2 L^2 \log (n r d A L/ (\epsilon\delta ) ))$, then with probability $1-\delta$, we have : for all $x\in {\cal P}$,
\begin{align*}
\left| g(x) - \sum_{i=1}^{3r} c_i \phi(w_i^\top S^\top S x - \theta_i) \right| < \epsilon \sup_{x\in {\cal P} } | g(x) |.
\end{align*}
\end{theorem}

\begin{proof}
The space $C[-1,1]$ is separable. That is, it contains a countable dense subset. Let $\{ u_m \}_{ m = 1 }^{\infty}$ be such a subset. We choose  $\{ u_m \}_{m=1}^{\infty}$ from among the set of all polynomials with rational coefficients. Then it is easy to see that each $u_m \in C^{\infty}[-1,1]$. Thus, to each $h \in C [ -1, 1]$ and each $\epsilon > 0 $ there exists a $k$ (dependent upon $h$ and $\epsilon$) for which
\begin{align*}
| h(t) - u_k(t) | < \epsilon, 
\end{align*}
for all $t\in [-1,1]$. 

Now, we can fix function $h$ and and integer $k$

We will now construct a strictly increasing $C^{\infty}$ sigmoidal function $\phi : [-\infty,+\infty] \rightarrow [0,1]$ with three properties

(\RN{1}) $\lim_{t \rightarrow - \infty} \phi(t) = 0$

(\RN{2}) $\lim_{t \rightarrow + \infty} \phi(t) = 1$

(\RN{3}) for each fixed $\epsilon > 0$, there exists real coefficients $a_{k,1}, a_{k,2}, a_{k,3}$ (depend on $h$ and $\epsilon$) and real offsets $b_{k,1} = -3, b_{k,2} = 1, b_{k,3} = 4k+1 $ such that
\begin{align*}
\left| h(t) - \sum_{i=1}^3 a_{k,i} \cdot \phi ( t + b_{k,i} ) \right| < \epsilon, \forall t \in [-1,1].
\end{align*}

 We do this by constructing $\phi$ so that 
\begin{align*}
\sum_{i=1}^3 a_{k,i} \cdot \phi ( t + b_{k,i} ) = u_{k}(t), 
\end{align*}
and $t \in [-1,1]$.

Let $f$ be any $C^{\infty}$, strictly monotone, sigmoidal function. There are many, for instance $f(t) = 1 / ( 1 + e^{-t} )$. We define $\phi$ on $[4m,4m+2]$, $m=1,2,\cdots,$ in the following way. Set $\phi ( t + 4m + 1 ) = c_m + d_m t+ e_m u_m(t)$ for $t \in [-1,1]$ where we choose the constants $c_m,d_m$ and $e_m$ so that
\begin{align*}
1. & ~ \phi(4m) = f(4m) \\
2. & ~ 0 < \phi'(t) \leq f'(t) \text{~on~} [4m,4m+2].
\end{align*}

 On the intervals $[-4,-2]$ and $[0,2]$ we require that function $\phi$ still satisfy conditions 1 and 2 in the above Equation. We also want $\phi (t-3)$ and $\phi (t+1)$ are linear function and also be linearly independent on $[-1,1]$. For example, we can choose
 \begin{align*}
\phi(t-3) = & ~ t - 3, \\
\phi(t+1) = & ~ t + 1.
 \end{align*}

 Finally, we can fill in the gaps in the domain of definition of $\phi$ (including all of $(-\infty,4)$) in such a way that $\lim_{t \rightarrow \infty} \phi(t) = 0$. 


According to the definition of $\phi$, for all $m =1,2,\cdots$, there exist reals $a_{m,1},a_{m,2},a_{m,3}$ and $b_{m,1}, b_{m,2}, b_{m,3}$ such that
\begin{align*}
\sum_{i=1}^3 a_{k,i} \phi (t + b_{k,i}) = u_k(t).
\end{align*}

Let $g\in {\cal R}_r$ and $\epsilon > 0$ be given. We may write
\begin{align*}
g (x) = \sum_{j=1}^r g_j (\alpha_j^\top \cdot x)
\end{align*}
for continuous function $g_j : [-1,1] \rightarrow \R$ and column vector $\alpha_j \in \R^n$ with $\| \alpha_j \|_2=1$, $j \in [r]$. From the above construction of $\phi$ there exist constants $\beta_{j,1}, \beta_{j,2}, \beta_{j,3}$ and an integers $\gamma_{j,1}=-3$, $\gamma_{j,2} = 1$ and $\gamma_{j,3}$ such that
\begin{align*}
\left| g_j(t) - \sum_{i=1}^3 \beta_{j,i} \phi ( t + \gamma_{j,i} ) \right| < \epsilon / r,
\end{align*}
for all $t\in [-1,1]$ and $j \in [r]$.

Replacing $t$ by $\alpha_j^\top x$, we have
\begin{align*}
\left|g_j (\alpha_j^\top x) - \sum_{i=1}^3 \beta_{j,i} \phi ( \alpha_j^\top x + \gamma_{j,i} ) \right| < \epsilon /r,
\end{align*}
for all $x \in B^n$, and hence
\begin{align*}
& ~ \left| g(x) - \sum_{j=1}^r \sum_{i=1}^3 \beta_{j,i} \phi (\alpha_j^\top x + \gamma_{j,i}) \right| < \epsilon,
\end{align*}
for all $x\in B^n$.

Choosing $S$ to be an oblivious neural subspace embedding matrix,
\begin{align*}
\left| g(x) - \sum_{j=1}^r \sum_{i=1}^3 \beta_{j,i} \phi (\alpha_j^\top S^\top S x + \gamma_{j,i}) \right| < \epsilon,
\end{align*}

 Now each $\phi (\alpha_j^\top x -3), \phi (\alpha_j^\top x +1), j\in [r]$, is a linear function, that is, a linear combination of $1,x_1,\cdots, x_n$. As such, the
\begin{align*}
\sum_{j=1}^r \beta_{j,1} \phi ( \alpha_j^\top  x - 3) + \beta_{j,2} \phi (\alpha_j^\top  x + 1), 
\end{align*}
may be rewritten using at most $n+1$ terms from the sum. This finishes the proof.

\end{proof}

